Modelo de Tratamiento para Tumores en Presencia de Radiaci\'on

In this work, we combine a new form of the cell survival fraction developed in [29] with the Gompertz cell growth model. The result is an equation that models the cell growth/death under a radiation dose and can be applied in a conventional radiation treatment (we chose conventional fractionation and hypofractionation). Later we optimize this equation in order to obtain the optimal doses that reduce the tumor's size or the number of cancer cells. We applied our results to breast cancer data: invasive ductal carcinoma (IDC) and ductal carcinoma in situ (DCIS)

==> capitulo1.tex <==
\section{Factores causantes de c\'ancer}

Como parte fundamental del desarrollo de estre trabajo, conviene saber algunas caracter\'isticas fundamentales del problema que estamos enfrentando. Por ello en el siguiente cap\'itulo describiremos los principios del proceso de inducci\'on al c\'ancer, el cual inicia con la aparici\'on de tumores malignos.

\section{C\'elulas cancer\'igenas y c\'ancer}

A lo largo de la existencia de un ser vivo, las c\'elulas de su organismo siguen un ciclo ordenado de divisi\'on y muerte celular. Este proceso de crecimiento es relativamente mas r\'apido durante su juventud. Al llegar a la etapa adulta el organismo continua con el proceso de divisi\'on a f\'in de reparar celulas "viejas" o dañadas. 
El c\'ancer es una enfermedad donde las c\'elulas del organismo comienzan un proceso de crecimiento descontrolado. Dicho crecimiento se debe a ciertos defectos de c\'elulas que en lugar de sufrir el proceso de apoptosis, tienden a replicarse y nuevas c\'elulas comienzan a desarrollarse. 

Las c\'elulas cancer\'igenas presentan caracter\'isticas muy diferentes a las c\'elulas sanas ya que continuan creciendo en n\'umero (sin morir), pueden llegar a formar masas de tejido anormal y continuan su replicaci\'on aunque el agente externo que lo provoc\'o haya desparacido. De igual modo, las c\'elulas cancerosas pueden transportarse por el organismo teniendo la capacidad de "contagiar" otros tejidos y diseminar la enfermedad. Una c\'elula sana se convierte en c\'elula cancer\'igena cuando ocurre una alteraci\'on en su ADN, interviniendo de manera directa en el proceso de replicaci\'on celular (crecimiento anormal y descontrolado). Si una c\'elula con el ADN alterado se replica, dar\'a lugar a copias id\'enticas con el ADN alterado. Este crecimiento anormal puede llevar a la formaci\'on de tumores si el n\'umero de c\'elulas cancer\'igenas es completamente grande. Cabe destacar que no todos los tumores son malignos, existen algunos considerados benignos. Los tumores benignos pueden ocasionar problemas dentro del \'area en que se desarrollan sin embargo no podr\'an diseminar la enfermedad (metastasis).  El cancer como enfermedad engloba a un todo conjunto de enfermedades clasificadas de acuerdo al tejido u \'organo que afectan \cite{25}.

Podemos englobar al c\'ancer dentro de los principales tres tipos que existen: los sarcomas, los carcinomas y las leucemias y linformas. Los sarcomas son tumores malignos provenientes de tejido conjuntivo (como huesos), muscular y vasos sanguineos. Los carcinomas son tumores formados a partir de tejido epitelial como la piel. Y por \'ultimo, la leucemia es un tipo de c\'ancer que afecta el proceso de producci\'on de leucocitos en la sangre mientras que los linfomas son tumores malignos de los ganglios linf\'aticos. 

\section{Factores causantes de c\'ancer}

Al d\'ia de hoy, las investigaciones sobre los factores que causan cancer continuan en pie. Durante este transcurso de tiempo se han podido indentificar diversos factores aunque se pueden resumir en dos tipos: factores hereditarios y factores externos. Los factores hereditarios se refieren al origen genetico del cancer por herencia. Existen genes llamados protooncogenes (que estimulan el crecimiento celular) y genes supresores tumorales que en condiciones normales previenen y regulan la replicaci\'on celular \cite{25}. Alguna falla dentro de este tipo de genes o incluso la ausencia de ellos, propician a que el individuo pueda desarrollar la enfermedad. Esta falla generalmente esta relacionada con las mutaciones en el ADN, la rotura de cromosomas y el traslado cromos\'omico \cite{25}.  

Dentro de los factores externos se incluyen: los factores qu\'imicos, agentes radiativos y las infecciones o virus. Los factores qu\'imicos provocan que la continua exposici\'on a esas sustancias provoquen daños a nivel celular, en la literatura existe todo un tratamiento de porqu\'e y c\'omo estos factores afectan el organismo, y a su vez la incidencia de los mismos \cite{25}. Los agentes radiativos son las radiaciones ionizantes, los fotones atraviesan la c\'elula y pueden provocar daño al ADN como rotura de los cromosomas. Entre menor sea la longitud de onda de dicha radiaci\'on existe un mayor riesgo de daño celular, es por ello que se utlizan rayos X en el tratamiento de tumores.
Las infecciones o virus pueden desecandenar la creacion y multiplicaci\'on de c\'elulas cancer\'igenas. Existen muchas evidencias que de distintos tipos de virus y bacterias estan relacionados con oncogenes y factores de crecimiento que estimulan el desarrollo de c\'elulas tumorales (para mas informaci\'on ver \cite{25}).


\section{Carcinog\'enesis}

A continuaci\'on describiremos el proceso de desarrollo del c\'ancer. 
Una c\'elula sana tiene la capacidad de convertirse en c\'elula cancer\'igena (cambiar su fenotipo) si es expuesta constantemente a un agente carcinogeno, de tal forma que se produzca una mutaci\'on del ADN. La c\'elula alterada puede replicarse si los mecanismos de supresion tumoral fallan. De este modo la celula maligna continua replicandose acumulando errores en cada etapa de duplicaci\'on, por lo que el riesgo para del desarrollo de la enfermedad es inminente. 

El proceso de carcinog\'enesis puede dividirse en tres etapas: \textbf{iniciaci\'on}, un cambio permanente y heredable que ocurren a nivel del ADN de la c\'elula; \textbf{promoci\'on}, etapa de crecimiento tisular que da lugar a la formaci\'on de tumores, por consecuencia de alteraciones gen\'eticas las c\'elulas alteradas proliferan y continuan acumulando daños; \textbf{progresi\'on}, cuando las c\'elulas cancer\'igenas continuan proliferando invadiendo tejidos adyacentes y metastizando otras partes del organismo \cite{26}.

Las c\'elulas tumorales presentan un consumo mayor de oxigeno, debido a ello contienen factores gen\'eticos que estimulan la angiog\'enesis tumoral \cite{25}. La angiogenesis tumoral esta relacionado a la continua proliferaci\'on de c\'elulas tumorales en el organismo (met\'astasis). Cabe destacar que una de cada diez mil c\'elulas que logre llegar al torrente sanguineo o el sistema linf\'atico, ser\'a capaz de desencadenar un cuadro de met\'astasis \cite{25,26}.  La met\'astasis generalmente es el proceso final de la enfermedad, cerda del 90\% de las muertes debidas a c\'ancer son debido a crecimientos de tumores en zonas alejadas del tumor primario (solo el 10\% se debe a tumores primarios) \cite{26}. 


\section{Tratamientos contra la enfermedad}

En general los m\'etodos de tratamiento que existen para combatir el c\'ancer son: cirug\'ia, radioterapia y quimioterapia. La cirug\'ia es el m\'etodo con mas historial y es usado para eliminar tumores tempranos localizados as\'i como en combinaci\'on de tratamientos. La quimioterap\'ia consiste en la aplicaci\'on de sustancias qu\'imicas antineoplasicas. Las sustancias atacan el ADN tanto de c\'elulas sanas como c\'elulas tumorales. De este modo se produce muerte celular de ambas partes. La radioterapia consiste en la aplicaci\'on de radiaci\'on ionizante en el area del tumor. La radiaci\'on afecta directamente al ADN de la c\'elula cancer\'igena provocandole la muerte. Cabe destacar que dependiendo del tipo de tumor se escoge el tratamiento adecuado. Algunos tumores requieren la utilizaci\'on del los tres tipos de tratamientos: radioterapia y/o quimioterapia para reducir el tamaño del tumor y finalmente cirug\'ia para extirparlo completamente del organismo. A partir de ahora nos enfocaremos en la utilizacion de la radiaci\'on como tratamiento. 

\subsection{Radioterapia Oncol\'ogica}

Como se mencion\'o anteriormente, la radioterapia consiste en la aplicaci\'on de radiaci\'on ionizante en el area del tumor. La radiaci\'on esta compuesta por flujos continuos de part\'iculas fermi\'onicas (electrones, protones o neutrones) o fotones.   Esta radiaci\'on se denomina ionizante debido a que tiene la capacidad de ionizar \'atomos con los que interactuan (arrancar electrones de ellos). Los electrones arrancados dentro de la c\'elula salen disparados y pueden llegar a interaccionar con otros electrones para arrancarlos de su orbital. Este proceso puede continuar a f\'in de ionizar mas \'atomos y llegar a formar clusters de ionizaci\'on \cite{21}. La radiaci\'on ionizante produce lesiones en las mol\'eculas de ADN y pueden provocar: ruptura de cadenas simples o dobles, alteraci\'on de las bases, destrucci\'on de azucares y formaci\'on de d\'imeros. Una vez que una c\'elula es alcanzada por una cantidad suficiente de radiaci\'on, se produce cualquiera de los daños descritos anteriormente. La c\'elula comienza el proceso de cit\'olisis: su membrana celular se descompone y pierde su capacidad de divisi\'on celular. Llegados a este punto podemos hablar de muerte celular como la perdida irreversible en la capacidad de reproducci\'on celular \cite{19}. La muerte celular, despues de un evento de radiaci\'on, se puede producir por diferentes tipos: apoptosis, autofagia, necrosis, senescencia (envejecimiento) celular y cat\'astrofe mit\'otica [21]. La mayoria de la muerte celular por radiaci\'on ionizante ocurre en etapas tardias de la cat\'astrofe mit\'otica y no inicialmente en respuesta a la radiaci\'on \cite{21}.   

Debido al complejo proceso que incluye el tratamiento de radiaci\'on es \'util definir t\'erminos como las dosis m\'aximas de radiaci\'on para un tejido, tiempos de recuperaci\'on y probabilidades de supervivencia celular. Estos conceptos ser\'an abordados con mas detalle en los cap\'itulos siguientes.  




%El proceso por el cual el organismo de alg\'un individuo llega al punto de formar tumores que conlleven a un diagn\'ostico de cancer es descrito en la literatura, as\'i como los factores externos que propician su desarrollo [21].
%Desde el comienzo de la investigaci\'on en c\'ancer se han observado crecimiento de tumores en laboratorios asi como %en pacientes, estas investigaciones han analizado desde la forma de los tumores hasta la rapidez con la que crecen o %se llegan a diseminar. 


==> capitulo11.tex <==
\chapter{Introducci\'on}

%\begin{Large}
%\section*{Interacci\'on tumor - sistema inmune}
%\end{Large}

%Los modelos matemáticos han sido ampliamente usados para describir
%el sistema inmune [4] y su interacción con las células tumorales, con y sin
%tratamiento. Estos modelos han sido usados para describir los efectos inmunodepresores
%del tumor [5], el papel del retraso de la respuesta del sistema inmune [6], tratamientos de radioviroterapia [7], %quimioterapia [8] e incluso cirugía [9]. El trabajo con estos modelos se basa sobre todo en la interacción del %tumor con el sistema inmune.

%El modelado matem\'atico y la simulaci\'on num\'erica de sistemas usando
%ordenadores es una herramienta que cuenta con casi 70 años de experiencia.
%Se utiliza habitualmente, por ejemplo, en los casos en los que la
%{experimentación es difícil (física de altas energías, etc.), cara y/o peligrosa
%(residuos tóxicos, nucleares, armamento) o en los casos en que se ven comprometidas
%vidas humanas (investigación en tratamientos oncológicos). El
%empleo masivo de ordenadores en las investigaciones científicas ha permitido
%trascender los temas estudiados por las llamadas “ciencias exactas” y
%realizar el modelado de fenómenos que parecían inalcanzables matemáticamente
%a los investigadores. Temas tales como los sistemas de muchas partículas,
%cálculos de modelos meteorológicos, rotura de estructuras, estructuras
%de proteínas y muchos más, constituyen hoy áreas de trabajo multidisciplinar
%donde colaboran activamente profesionales de las más diversas ramas. Los
%resultados de estos enfoques han dado lugar a una nueva concepción de
%los métodos de investigación y hasta de la propia estructura y contenido de
%las ciencias [1]. Ha surgido una interdisciplinariedad del conocimiento que
%difícilmente era previsible a mediados del siglo pasado. En unos pocos años
%han brotado nuevas ramas del conocimiento como la física de los sistemas
%complejos, la bioinformática, la ciencia del caos, etc. con una penetración
%insospechada en la estructura conceptual del resto de las ciencias e incluso
%de la sociedad como en el caso de la sociofísica y la econofísica. Durante
%las últimas décadas se ha puesto de manifiesto que el modelado y el estudio
%cualitativo de los sistemas dinámicos [2] nos ha permitido avanzar en el
%entendimiento de muchos sistemas, entre ellos algunos sistemas biológicos [3].

%El sistema inmune, como todo sistema de respuesta defensivo, se encuentra diseñado
%para reconocer y destruir estructuras extrañas y respetar los tejidos propios. La base
%de este complejo sistema se encuentra en el denominado sistema mayor de histocompatibilidad
%(HLA). Las moléculas de este sistema son glicoproteínas que se encuentran situadas 
%en la membrana celular. Existen dos tipos de HLA (clase I y II). El primero se encuentra
%en todas las células nucleadas del organismo. Es específico de cada individuo y está 
%diseñado sólo para unirse y presentar en la superficie celular péptidos de la célula.
%Son reconocidos como propios por lo que no se desencadena una respuesta inmune. 
%Únicamente cuando las células se encuentran parasitadas por virus o se transforman en
%neoplásicas, producen moléculas con epítopos para los cuales el sistema inmune no es
%tolerante, son reconocidos por los linfocitos T citotóxicos (CD8) y destruidas. El 
%sistema HLA clase II sólo se encuentra en la superficie de las células presentadoras
%de antígenos, es decir, en los linfocitos B, células dendríticas y células de estirpe
%monocito/ macrófago. Cuando un antígeno penetra en el organismo es captado por estas
%células y, en los lisosomas, se une a la proteína HLA tipo II que se ha sintetizado
%en el retículo endoplasmático. La variabilidad de esta proteína hace que sólo pueda
%unirse con aquellos antígenos que encajen en su hendidura. Cuanto mejor encajen mayor
%afinidad tendrá por ellos. De este modo, este complejo sale a la superficie de la 
%célula, siendo el antígeno presentado a los linfocitos colaboradores o CD4 que ponen
%en marcha la respuesta inmune. Este es un paso fundamental del sistema, si un antígeno
%no puede unirse a una proteína HLA, éste no podrá ser presentado y no existirá 
%respuesta inmune [10].

%\vspace{3pt}

%\begin{figure}[h!]
%    \centering
%    \includegraphics[scale=0.54]{cmh}
%    \caption{Procesamiento y presentaci\'on de ant\'igenos ex\'ogenos por una c\'elula presentadora de %   %   % %     ant\'igenos}
%    \label{g2}
%   \end{figure}

%El cáncer es un grupo de enfermedades que se caracterizan por la presencia
%de células sin el mecanismo de apoptosis o muerte celular. Este grupo
%de células puede crecer indefinidamente y afecta al resto de células del organismo
%al consumir los nutrientes y el espacio destinadas a ellas. La aparición
%de estos grupos de células cancerígenas desencadena una respuesta inmune
%en el organismo. Los linfocitos se enlazan a las células tumorales creando
%complejos conjugados o de asociación, que pueden terminar programando
%las células tumorales para morir o con la desactivación de los linfocitos. Este
%proceso puede ser suficiente para destruir el tumor si la respuesta del sistema
%inmune es adecuada. El cáncer como enfermedad aparece cuando la
%respuesta del sistema inmune es insuficiente para detener el proceso y es
%necesario acudir a un tratamiento externo.
%La cirugía y la radioterapia son los tratamientos más efectivos contra el
%cáncer. La cirugía no sólo tiene una más antigua tradición, sino que constituye
%en la mayoría de los casos, la forma primaria de tratamiento y es la que,
%para tumores no metastásicos, alcanza un mayor porcentaje de resultados
%positivos. La radioterapia, sin embargo, se ha desarrollado enormemente y
%no sólo ayuda a erradicar muchos tumores sino que puede utilizarse, junto
%con la cirugía, en su control a a largo plazo [11].
%La dificultad de realizar estudios sobre seres vivos con variaciones en las
%dosis, tiempo de aplicación y tiempos entre secuencias, hace del modelado
%numérico la herramienta idónea para estudiar el comportamiento de la evolución
%temporal del tumor. No obstante, estos métodos de estudio, encuentran
%siempre un escollo al intentar aplicarse clínicamente, ya que, el gran número
%de variables presentes hace muy difícil aplicar los resultados a un paciente
%determinado. Aún así, realizando un estudio estadístico de los resultados
%de las simulaciones, es posible disminuir la cantidad de parámetros a tratar.
%Junto a los datos existentes de pacientes reales, o nuevos análisis clínicos
%propuestos por oncólogos, debería ser posible ajustar estos modelos matemáticos
%a casos clínicos y predecir, estadísticamente, los resultados de un
%tratamiento de radioterapia.

%\vspace{40mm}
%\begin{Large}
%\section*{Modelos de crecimiento tumoral}
%\end{Large}

%En [20] se introdujo la influencia de radiación en el desarrollo de tumores regidos por las ecuaciones:

%\begin{equation}
%    \begin{array}{cl}
%        \dot{X} =& aX-bXY  \\
%        \dot{Y} =& d XY-fY-kX+u 
%    \end{array} 
%\end{equation}

%Siendo $X$ la población de células cancerosas, $Y$ la poblacion de celulas que interactuan con las c\'elulas %cancerosas a fin  de tratar de eliminarlas; $a$, $b$ ,$d$ ,$f$  los coeficientes de proporcionalidad que entran %en los modelos de Lotka-Volterra; $u$ el flujo de linfocitos que envia el organismo a la zona afectada por el %tumor y $kX$ un término de inmunodepresión del tumor. Los resultados obtenidos son muy buenos en términos de %predicción, aunque este modelo tiene aspectos discutibles como la presencia de linealidad en el término de %inmunodepresión, la constancia de u, etc.

%Un estudio más práctico, en t\'erminos de predicci\'on, consistir\'ia en  introducir el modelo de Gompertz para %el crecimiento de tumores, el cual es conocido en la comunidad médica, introduciendo la influencia de la %radiación mediante un modelo de supervivencia tisular.

%Los modelos de crecimiento poblacionales han sido \'utiles para la descripcion del crecimiento (respecto del  %tiempo) de, entre otras cosas, organismos vivos. Debido a ello se populariz\'o  su uso en problemas relacionados %al crecimiento de c\'elulas. Existen diferentes tipos de modelos de crecimiento de c\'elulas (para este caso %describir\'an c\'elulas cancer\'igenas, los parametros de la ecuaci\'on nos dir\'an que es lo que describe el %modelo) basados en diferentes premisas como, el comportamiento de la c\'elula a lo largo del tiempo,  si es %coherente con relaciones alom\'etricas o no, etc.

%Para el presente trabajo se considerar\'a de relevancia el modelo de Gompertz ya que dicho modelo describe un %crecimiento lento al inicio y el final del periodo de tiempo, lo cual sucede realmente en diferentes tipos de %tumores [21].

%Los modelos tipo Gompertz son modelos emp\'iricos para el crecimiento de sistemas biologicos. Existen  diferentes %tipos de modelos de Gompertz los cuales ajustan con la informaci\'on cl\'inica: existe un tama\~no limite para el %crecimiento de un tumor respecto del tiempo [21,24]. Podemos enumerar los diferentes tipos de ecuaciones de %Gompertz, todas ellas difieren solo por los parametros que se consideran. 

%\section*{Modelo Generalizado de Dos Par\'ametros}

%En este caso se considera que la tasa de cambio en el n\'umero de c\'elulas cancer\'igenas es una diferencia %entre la tasa de crecimiento y la tasa de degradaci\'on (muerte celular). Adem\'as la tasa de cambio es %proporcional al tama\~no del tumor [23] 

%\begin{equation}
%    \frac{dx}{dt}=ax^{\alpha}-bx^{\beta} \tag{2}
%\end{equation}

%donde $x=x(t)$ es el n\'umero de c\'elulas cancer\'igenas en un instante $t$ y $a,b,\alpha, \beta$ son parametros %relacionados con la tasa de crecimiento.  Particularmente si $\alpha=\beta$ obtenemos el llamado modelo de %Gompertz generalizado

%\begin{equation}
%    \frac{dx}{dt}=ax^{\alpha}-bx^{\alpha}\text{ln}x \tag{3}
%\end{equation}

%si $\alpha=1$ obtenemos el modelo de Gompertz

%\begin{equation}
%    \frac{dx}{dt}=ax-bx\text{ln}x \tag{4}
%\end{equation}

%\section*{Modelo Gen\'erico}

%En este tipo de modelo se supone que la tasa de cambio del n\'umero de c\'elulas es proporcional a una funci\'on %que incrementa con el tama\~no y otra que disminuye con el tama\~no

%\begin{equation}
%    \frac{dx}{dt}=\frac{r}{N^n}x^{1-np} (N^n -x^n)^{1+p} \tag{5}
%\end{equation}

%donde $N$ es la cap\'acidad m\'axima de carga (el tamaño m\'aximo que puede alcanzar el tumor) y $r,n,p$ %constantes relaxionadas con la tasa de crecimiento. De manera an\'aloga, si $n=0$, obtenemos el modelo llamado %Hyper-Gompertz \cite{33}

%\begin{equation}
%    \frac{dx}{dt}= r x \left( \text{ln} \frac{N}{x} \right)^{1+p} \tag{6}
%\end{equation}

%Si en la ecuaci\'on anterior $p=0$ obtenemos de nuevo el modelo de Gompertz 

%\begin{equation}\label{eq12}
%    \frac{dx}{dt}=r x \text{ln}\frac{N}{x} \tag{7}
%\end{equation}

%Hay que destacar que todos estos modelos son equivalentes respecto de su comportamiento en el crecimiento, la %elecci\'on de uno u otro depender\'a del analisis que se lleve a cabo.

%\begin{Large}
%\section*{Supervivencia celular frente a la radiación}
%\end{Large}

%El efecto de la radiación ionizante sobre tejidos biológicos da lugar a procesos
%que difieren enormemente en cuanto a la escala de tiempos en que ocurren. Estos procesos se dividen en tres %fases. La primera o fase física,
%consiste en las interacciones de las partículas cargadas y los átomos que
%componen el tejido. Un electrón de alta energía atraviesa la molécula de ADN
%en $10^{-18}$ segundos y una célula en alrededor de $10^{-14}$ segundos. Al interaccionar
%con los electrones orbitales los desprende de los átomos (ionización)
%y eleva a otros a un nivel más alto de energía (excitación). Si tienen suficiente
%energía, estos electrones secundarios, pueden excitar o ionizar otros átomos
%a su paso, dando lugar a una cascada de eventos de ionización.
%La fase química toma lugar inmediatamente después y describe el período
%en el cual estos átomos y moléculas excitados reaccionan con otros
%componentes celulares en rápidas reacciones químicas. En esta etapa se
%rompen los enlaces químicos y se crean radicales libres. Estos son altamente
%reactivos y provocan una sucesión de reacciones que conducen, en su
%momento, a la restauración del equilibrio electrónico de la célula. Estas reacciones
%de los radicales libres tienen lugar en el primer milisegundo de exposición
%a la radiación.

%Todos los demás procesos se engloban en la última fase, la fase biológica.
%Esta comienza con reacciones enzimáticas que actúan sobre el daño
%químico residual. Se reparan la gran mayoría de las lesiones satisfactoriamente
%pero algunas de estas reparaciones fallan y conducen a la muerte
%celular. Las células no mueren inmediatamente e incluso en caso de una
%pequeña exposición a la radiación, pueden realizar determinado número de
%divisiones mitóticas antes de hacerlo. En la última etapa de los efectos irradiación
%pueden aparecer las reacciones tardías, como la fibrosis o el daño
%en la médula espinal.
%Estos efectos de la radiación pueden agruparse, según la escala de tiempos
%en que se desarrollan, en instantáneos para aquellos que ocurren en una escala de tiempos muy pequeña (fases %física y química) y tardíos para aquellos que ocurren en la última etapa de reacción a la radiación (reacciones %tardías de la fase biológica).

%Existen varios modelos matemáticos que intentar explicar la interacción
%de la radiación con la materia y que agrupan los procesos que tienen lugar en
%el período temprano y que expondremos a partir de la detallada recopilación
%que puede encontrarse en [19].


%El más simple es el modelo lineal que plantea que cada partícula ionizante
%que atraviesa la célula provoca un evento letal. La producción de eventos
%letales es aleatoria y su número se incrementa en proporción directa a la dosis
%de radiación. La fracción de supervivencia de las células es una función
%exponencial de la dosis, descrita por un proceso de Poisson. De modo que,

%\begin{equation}
%    F_{s}=exp[-\alpha D] \tag{8}
%\end{equation}

%donde D es la dosis de radiación absorbida,  $\alpha$  un coeficiente de proporcionalidad
%y $F_s$ es la fracción de células que sobreviven al proceso. En términos
%biológicos esto significa que un único impacto es capaz de matar a la célula.
%Otros modelos están dedicados al mejoramiento empírico de fórmulas de supervivencia para mejorar el ajuste con %los datos experimentales. [11- 19]. En [20] se propuso un modelo estadístico basado en la extremización de la %entropía de Tsallis, que arroja excelentes resultados al comparar la fracción de supervivencia tisular calculada %por este método, con los experimentos. A grandes rasgos, su fundamento es el siguiente:

%La mecánica estadística clásica se basa en el axioma de que la interacción
%entre las diferentes partes de un sistema es, al menos, muy débil. Esto
%es, que los subsistemas que componen el sistema a estudiar son independientes
%o tienen una correlación débil. La definición de entropía de Boltzmann-Gibbs (BG) es
%extensiva bajo estas condiciones. No obstante, si las diferentes partes del
%sistema estudiado están fuertemente correlacionados, la entropía de BG no
%puede aplicarse. Debe entonces buscarse una nueva definición de entropía
%que tome en cuenta las interacciones no triviales entre los componentes del
%sistema pero que al mismo tiempo tienda a la entropía de BG en el límite
%extensivo.

%Si consideramos
%cuidadosamente el efecto de la radiación sobre la materia viva, vemos que
basta una cantidad finita de radiación para eliminar todas las células. Para
aplicar el principio de máxima entropía pediremos que exista una cantidad
determinada de radiación absorbida o su efecto tisular equivalente,
tal que ninguna célula sobreviva a este efecto tisular (algo no contemplado
en los modelos radiobiológicos pero constatado por la experiencia
clínica).
Usaremos la entropía de Tsallis [40]:

\begin{equation}
    S_q = \frac{1}{q-1} \left( 1-\int_{0}^{\infty} p^q (E)dE \right)=\frac{1}{q-1}\left( 1-\int_{0}^{\Omega} p^q (E)dE \right) \tag{9}
\end{equation}

como la entropía generalizada, donde q es un coeficiente que caracteriza la
no extensividad del fenómeno. Puede demostrarse que la entropía de Tsallis
se reduce a la de BG cuando el parámetro de no extensividad  tiende a 1 ($q \rightarrow 1$). En
este sentido, la entropía de Tsallis puede considerarse como una generalización
de la entropía de BG y puede aplicarse en problemas donde no puede
aplicarse la entropía de BG (sistemas con correlaciones de largo alcance,
memoria, etc.) [38]. El problema de la radiación en los tejidos vivos es un buen ejemplo de estos problemas.

A su vez, puede obtenerse una forma diferente para la fracción de supervivencia de c\'elulas bajo una dosis de radiaci\'on \cite{20}:

\begin{equation}
    F_s (E)=\left( 1-\frac{E}{\Omega} \right)^{\frac{2-1}{1-q}} \tag{10}
\end{equation}

siendo $E$ el llamado efecto tisular y $\Omega$ el "efecto tisular límite", por  encima del cual $F_s (E)=0$ . Expresado en funcion de la dosis $D$, sería:

\begin{equation}
    F_s (D)= \left\{
    \begin{array}{cc}
        (1-\frac{D}{\Delta})^\gamma & \forall D < \Delta \\
         0 & \forall D \geq \Delta 
    \end{array}
    \right. \tag{11}
\end{equation}

donde $\gamma=\gamma(q)$ , y $\Delta$  es la radiación mínima letal.
El valor de $\Delta$  define un punto crítico para la probabilidad de supervivencia
de las células. Para $D < \Delta$  las probabilidades de supervivencia y muerte
coexisten pero cuando $D$ se iguala a $\Delta$ , tiene lugar una “transición de fase”
y ninguna célula es capaz de sobrevivir. 
Aunque la fracción de supervivencia celular $F_s$ como función de $D$ depende
de múltiples factores, como la tasa de dosis o el tipo de radiación, la dependencia de $F_s$ con ($1-D/\Delta$)   tiene un carácter universal. Por supuesto, todo esto ser\'a tratado con mayor detalle en los cap\'itulos siguientes. 
El parámetro fundamental es entonces el exponente, que depende del valor de q, el cual divide el comportamiento celular en clases de universalidad tal y como ocurre en los
fenómenos críticos.
La ecuación obtenida presenta la dificultad conceptual de que la aditividad de las dosis no conlleva la independencia estadística, lo que hace pensar que las dosis no son aditivas o sea $F_s (D_1 + D_2) \neq F_s (D_1) + F_s (D_2)$  lo cual debe tomarse en cuenta.

\newpage

\begin{Large}
\section*{Objetivos}
\end{Large}

Ahora podemos recapitular sobre la necesidad de tener un modelo de crecimiento combinando resultados para una fracci\'on de supervivencia celular (de un tejido). Recordemos que los modelos de crecimiento describen el proceso de crecimiento celular (tama\~no del tumor) sin ning\'un de proceso de control, es decir, como el tumor crecer\'ia a lo largo del tiempo sin intervencion de agentes externos (medicamentos, radiacion, etc). 
El an\'alisis planteado conlleva a ciertas restricciones en el problema, como la maximizaci\'on sobre el da\~no ocasionado a las c\'elulas cancer\'igenas y la minimizaci\'on del da\~no a c\'elulas sanas, los intervalos en la cantidad de radiaci\'on soportada por un paciente, la fracci\'on de c\'elulas que sobreviven a un evento radiativo, etc. Hablamos, entonces, de una restricci\'on en la dosis de radiaci\'on. En la literatura existen modelos de crecimiento bajo dosis de radiacion [20,22] pero la fracci\'on de supervivencia celular se toma como una funci\'on exponencial de la forma

\begin{equation}
        F_s (D)= e^{-D/<D>} \tag{12}
\end{equation}

con $<D>$ la dosis media. No obstante este modelo de la fracci\'on de supervivencia solo ajusta para dosis de radiaci\'on baja y algunos tejidos [21]. Como se menciono anteriormente, un estudio del modelo de crecimiento de Gompertz con la introducci\'on del modelo de supervivencia celular expuesto en [21] resultar\'ia mas pr\'actico e interesante.






